Understanding or Manipulation: Rethinking Online Performance Gains of Modern Recommender Systems

Recommender systems are expected to be assistants that help human users find relevant information automatically without explicit queries. As recommender systems evolve, increasingly sophisticated learning techniques are applied and have achieved better performance in terms of user engagement metrics such as clicks and browsing time. The increase in the measured performance, however, can have two possible attributions: a better understanding of user preferences, and a more proactive ability to utilize human bounded rationality to seduce user over-consumption. A natural following question is whether current recommendation algorithms are manipulating user preferences. If so, can we measure the manipulation level? In this paper, we present a general framework for benchmarking the degree of manipulations of recommendation algorithms, in both slate recommendation and sequential recommendation scenarios. The framework consists of four stages, initial preference calculation, training data collection, algorithm training and interaction, and metrics calculation that involves two proposed metrics. We benchmark some representative recommendation algorithms in both synthetic and real-world datasets under the proposed framework. We have observed that a high online click-through rate does not necessarily mean a better understanding of user initial preference, but ends in prompting users to choose more documents they initially did not favor. Moreover, we find that the training data have notable impacts on the manipulation degrees, and algorithms with more powerful modeling abilities are more sensitive to such impacts. The experiments also verified the usefulness of the proposed metrics for measuring the degree of manipulations. We advocate that future recommendation algorithm studies should be treated as an optimization problem with constrained user preference manipulations.

==> papers/4-solution.tex <==
\section{A Simple Solution To Alleviate Manipulation}

We have seen manipulation in both slate and sequential recommendations in the above sections and it is worth noting that manipulation could produce adverse effects towards both individuals and the society.
For users, their click or purchase caused by manipulation is contrary to their initial preference and will reduce their consuming experience in the long run.
For the society, manipulation will cause a loss of diversity and social homogenization, which runs counter to the original intent of the recommender system.
In order to alleviate manipulation, we propose a simple solution. Note that we do not model the decoy effect very thoroughly and it's just a first step to shed light on a possible way to alleviate manipulation.

\begin{align}
    c_{ijk} &= w_k r_{j} \exp(r_j-r_i) \label{eq:cijk}
\end{align}

We model user's click probability through Eq.\ref{eq:cijk}, where $c_{ijk}$ stands for the click probability of item $j$ when item $j$ is placed on the $k^{th}$ position and item $i$ is placed on the $k-1^{th}$ position. 
Through the observation of our dataset, we consider that user's click probability $c_{ijk}$ consists of three parts, namely the position bias, the predicted relevance of 
item $j$ towards the user and the decoy effect.
To be specific, $w_{k}$ stands for the position bias when an item is placed on the $k^{th}$ position, it is estimated by several rounds of random interact with a small amount of users. $r_{j}$ is the predicted relevance of item $j$ towards the user. $\exp(r_j-r_i)$ stands for the influence of decoy effect on item $j$. 
The estimation of decoy effect is simplified here by just taking into account the adjacent items and we model the decoy effect through an exponential distribution.
That is to say, when the predicted relevance of previous item $i$ is lower than that of item $j$, then $\exp(r_j-r_i)$ is greater than one, so it contributes positively to the click probability, on the contrary, when the predicted relevance of previous item $i$ is higher than that of item $j$, then $\exp(r_j-r_i)$ is less than one and it will contribute negatively to the click probability.
In our experiment, we multiply $w_{k}$ and $\exp(r_j-r_i)$ and take its inverse as a weight to reweight the loss function in the training process in order to alleviate manipulation.

